Integrating prediction in mean-variance portfolio optimization

Prediction models are traditionally optimized independently from their use in the asset allocation decision-making process. We address this shortcoming and present a framework for integrating regression prediction models in a mean-variance optimization (MVO) setting. Closed-form analytical solutions are provided for the unconstrained and equality constrained MVO case. For the general inequality constrained case, we make use of recent advances in neural-network architecture for efficient optimization of batch quadratic-programs. To our knowledge, this is the first rigorous study of integrating prediction in a mean-variance portfolio optimization setting. We present several historical simulations using both synthetic and global futures data to demonstrate the benefits of the integrated approach.

==> a__prop_8.tex <==

\subsection{Proof of Proposition \ref{prop:eqcon_tracking_error} }
Let $\bz^*(\toi{\by})$ and $\bz^*(\toi{\hat{\by}})$ be as defined in Equation $\eqref{eq:mvo}$ and Equation $\eqref{eq:z_star_uncon}$, respectively. Recall, the objective function of the minimum-tracking representation of the IPO program is:
\begin{equation} \label{eq_a:uncon_tracking_error_obj}
L_{\text{te}}(\btheta) = \frac{1}{2m} \sum_{i = 1}^m \lVert \bz^*(\toi{\hat{\by}}) - \bz^*(\toi{\by})  \rVert^2_{\toi{\bV}}
\end{equation}
The first-order necessary conditions for optimality of Program $\eqref{eq:mvo}$ state:
\begin{equation}\label{eq_a:mvo_fonc}
 \toi{\bV} \bz^*( \toi{\by} ) =  \toi{\by}
\end{equation}
Expanding  Equation $\eqref{eq_a:uncon_tracking_error_obj}$ and substituting in Equation $\eqref{eq_a:mvo_fonc}$  completes the proof:
\begin{equation} \label{eq_a:uncon_tracking_error_obj}
\begin{split}
L_{\text{te}}(\btheta) & = \frac{1}{2m} \sum_{i = 1}^m \big( \bz^*(\toi{\hat{\by}}) - \bz^*(\toi{\by}) \big)^T \toi{\bV} \big( \bz^*(\toi{\hat{\by}}) - \bz^*(\toi{\by}) \big)\\
& =  \frac{1}{m} \sum_{i = 1}^m   \frac{1}{2} \bz^*(\toi{\hat{\by}})^T \toi{\bV} \bz^*(\toi{\hat{\by}}) -\bz^*(\toi{\hat{\by}})^T \toi{\bV}\bz^*(\toi{\by})  + \frac{1}{2} \bz^*(\toi{\by})^T \toi{\bV} \bz^*(\toi{\by}) \\
& =  \frac{1}{m} \sum_{i = 1}^m   \frac{1}{2} \bz^*(\toi{\hat{\by}})^T \toi{\bV} \bz^*(\toi{\hat{\by}}) -\bz^*(\toi{\hat{\by}})^T\toi{\by}  + \bz^*(\toi{\by})^T \toi{\bV} \bz^*(\toi{\by}) .
\end{split}
\end{equation}





==> b_a_method.tex <==
\section{Methodology}\label{sec:method}
We begin by formally defining the traditional `predict, then optimize' framework which will help draw the distinction to the IPO alternative. We assume that we have a  cost function $c \colon \mathbb{R}^{d_z} \times \mathbb{R}^{d_y} \to \mathbb{R}$, which takes as input a decision vector $ \bz \in \mathbb{R}^{d_z}$ constrained to a feasible region $\mathbb{S} \subseteq \mathbb{R}^{d_z}$,  and a quantity of interest $ \toi{\by} \in \mathbb{R}^{d_y}$. If the realization $  \toi{\by}$ is known then generating optimal decisions amounts to solving the following deterministic optimization problem:

\begin{equation} \label{eq:pd}
\begin{split}
\minimize_{ \bz \in \mathbb{S}}   c( \bz,   \toi{\by}),
\end{split}
\end{equation}
with optimal solution:
\begin{equation} \label{eq:pd_sol}
\begin{split}
 \bz^*(  \toi{\by}) &  = \argmin_{  \bz \in \mathbb{S}}  c(  \bz,   \toi{\by}).
\end{split}
\end{equation}

In reality, we do not know the true value of $  \toi{\by}$ at decision time. We therefore estimate the values $  \toi{\by}$ through associated feature variables $  \toi{\bx} \in \mathbb{R}^{d_x}$. We define a prediction model by the function $f\colon \mathbb{R}^{d_x} \times \mathbb{R}^{d_\theta} \to \mathbb{R}^{d_y}$, where $f$ belongs to the class of regression models  $\mathbb{F} = \{f \mid f( \bx,  \btheta) =  \btheta^T   \bx\}$ and the parameter $  \btheta$ is constrained to the feasible region $ \bTheta \subseteq \mathbb{R}^{d_\theta}$. For a particular $  \btheta$, we define the estimate $\toi{\hat{\by}}$ as:
\begin{equation} \label{eq:yhat}
    \toi{\hat{\by}} = f(  \toi{\bx},  \btheta)  =  \btheta^T  \toi{\bx} .
\end{equation}

In traditional parameter estimation, $ \btheta$ would be chosen in order to minimize a prediction-based loss function $\ell \colon \mathbb{R}^{d_y} \times \mathbb{R}^{d_y} \to \mathbb{R}$, such as least-squares or negative log-likelihood. Specifically, given training data set $ D = \{(  \toi{\bx},  \toi{\by})\}_{i=1}^m$ we choose $\hat{  \btheta}$ such that:

\begin{equation} \label{theta_hat}
\begin{split}
    \hat{ \btheta} = \argmin_{  \btheta \in  \bTheta}  \mathbb{E}_D[\ell (f( \toi{\bx},  \btheta),  \toi{\by})],
\end{split}
\end{equation}
where $\mathbb{E}_D$ denotes the expectation operator with respect to the training distribution $D$. Once $\hat{ \btheta}$ has been determined, a traditional `predict, then optimize' framework, would then `plug-in' the estimate, $\toi{\hat{\by}}$, into program $\eqref{eq:pd}$ in order to generate the optimal decisions $ \bz^*(\toi{\hat{\by}})$.
%= f( \toi{\bx},  \hat{ \btheta})

In this paper, we are interested in optimizing $  \btheta$ in the context of the  cost, $c$, and its constraints, $\mathbb{S}$, in order to minimize the average realized  cost of the policy $ \bz^*( \toi{\bx},  \btheta)$ induced by this parameterization. For a fixed instantiation  $( \toi{\bx}, \btheta)$, we solve the decision program $\eqref{eq:pc}$ in order to determine the optimal action $ \bz^*( \toi{\bx},  \btheta)$ corresponding to our observed input $ \toi{\bx}$. Specifically, we solve:
\begin{equation} \label{eq:pc}
\begin{split}
\minimize_{ \bz \in \mathbb{S}}  c( \bz, f( \toi{\bx},  \btheta) ),
\end{split}
\end{equation}
with optimal solution given by:
\begin{equation} \label{eq:pc_sol}
\begin{split}
  \bz^*( \toi{\bx}, \btheta) &  = \argmin_{ \bz \in \mathbb{S}}  c( \bz,  f( \toi{\bx},  \btheta) ).
 \end{split}
\end{equation}
Our objective is to therefore choose $ \btheta$ in order to minimize the average realized  cost induced by the decision policy $ \bz^*( \toi{\bx},  \btheta)$. The resulting integrated prediction-optimization problem is a stochastic optimization problem, presented in program $\eqref{eq:ed2}$.
\begin{equation} \label{eq:ed2}
\begin{split}
\minimize_{ \btheta \in  \bTheta} \quad & \mathbb{E}_D[ c( \bz^*(  \bx,  \btheta), \by) ] \\
\text{subject to }\quad  &    \bz^*( \bx,  \btheta)  = \argmin_{ \bz \in \mathbb{S}}  c( \bz,  f( \bx,  \btheta) ).
\end{split}
\end{equation}
In practice, we are typically presented with discrete observations $ D = \{( \toi{\bx}, \toi{\by})\}_{i=1}^m$ and therefore we can approximate the expectation by its sample average approximation \citep{Shapiro2009}. The full IPO problem is presented in discrete form in program $\eqref{eq:erm}$:
\begin{equation} \label{eq:erm}
\begin{split}
\minimize_{ \btheta \in \bTheta} \quad & \frac{1}{m} \sum_{i=1}^m c(\bz^*(\toi{\bx}, \btheta), \toi{\by})  \\
\text{subject to }\quad  &   \bz^*(\toi{\bx}, \btheta)  = \argmin_{\bz \in \mathbb{S}}  c(\bz,  f(\toi{\bx}, \btheta) ) \quad \forall i \in 1,...,m.
\end{split}
\end{equation}
Note that program $\eqref{eq:erm}$ resembles the well documented empirical risk minimization \citep{Vapnik1992}, where the objective is to choose $\btheta$ in order to minimize the average empirical  cost. The notable difference, of course, is that for a fixed instantiation $\btheta$, the decision policy, $\bz^*(\toi{\bx}, \btheta)$, is optimal in the context of its decision program, which assumes predictions of the form $\toi{\hat{\by}} = f(\toi{\bx}, \btheta)$.

The IPO formulation results in a complicated dependency of the model parameters, $\btheta$, on the optimized values, $\bz^*(\toi{\bx}, \btheta)$, connected through the $\argmin$ function. This problem is frequently encountered in modern machine learning applications and there are several approaches for overcoming this challenge. For example, the problem can be structured as a bi-level optimization problem in which, under special constraint cases, an analytical solution for the gradient exists \citep{Gould2016}. Alternatively, heuristic methods, such as the one provided by \citet{Sinha2020},  propose structuring the problem as a bi-level optimization and use kriging (Gaussian process models) to approximate the mapping to the lower-level optimization problem.

In Section \ref{sec:mvo}, we discuss this relationship more fully in the context of mean-variance optimization. We first consider the general problem whereby the MVO  program contains both linear equality and inequality constraints. We follow  \citet{Amos2017} and \citet{Donti2017} and provide the current state-of-the-art formulation that re-structures the problem as an end-to-end trainable neural network with a differentiable quadratic programming layer and optimizes the prediction model parameters by gradient descent. We then consider several special cases, in which an analytical solution to the MVO program  exists, and discuss in detail the theoretical properties and practical benefits of the IPO estimator.


%First, in the case where the  program is either unconstrained or contains only linear equality constraints, then an analytical solution exists and is provided for both univariate and multivariate regression.  For the more difficult case where the  program includes linear inequality constraints, we follow \citet{Amos2017} and \citet{Donti2017} and re-structure the problem as an end-to-end neural network with a differentiable quadratic programming layer. With appropriate Hessian information, the neural network formulation is capable of solving the unconstrained and linear equality constrained IPO problems in a single Newton step, which is the approach used in practice. For the general inequality constrained case, we make use of stochastic gradient descent for locally solving the IPO problem.








